Advances in Automatically Rating the Trustworthiness of Text Processing Services

AI services are known to have unstable behavior when subjected to changes in data, models or users. Such behaviors, whether triggered by omission or commission, lead to trust issues when AI works with humans. The current approach of assessing AI services in a black box setting, where the consumer does not have access to the AI's source code or training data, is limited. The consumer has to rely on the AI developer's documentation and trust that the system has been built as stated. Further, if the AI consumer reuses the service to build other services which they sell to their customers, the consumer is at the risk of the service providers (both data and model providers). Our approach, in this context, is inspired by the success of nutritional labeling in food industry to promote health and seeks to assess and rate AI services for trust from the perspective of an independent stakeholder. The ratings become a means to communicate the behavior of AI systems so that the consumer is informed about the risks and can make an informed decision. In this paper, we will first describe recent progress in developing rating methods for text-based machine translator AI services that have been found promising with user studies. Then, we will outline challenges and vision for a principled, multi-modal, causality-based rating methodologies and its implication for decision-support in real-world scenarios like health and food recommendation.

==> content/part1_talk_cv.tex <==
\subsection{Part I: Talk and CV}
% --------------------
\section{Talk Outline }

The proposed talk intends to introduce and discuss the main research questions for assessing and assigning trust labels (rating) to Artificial Intelligence (AI) systems in a black box setting.  The proposed talk outline  topics that are described in more details in the
attached paper.

\begin{enumerate}
    \item Motivation and vision
    \begin{itemize}
        \item Black-box settings: no access to code or data
        \item Testing AI in black-box setting via data perturbation
        \item Communicating their risks via labels
    \end{itemize}
    \item The problem of trust in AI - omission and commission
    \begin{itemize}
        \item Data supply chains, lack of diversity
        \item Model supply chains
        \item By commission - adversary triggered attacks
    \end{itemize}
    \item Promoting trust via {\em Transparency through documentation}
    \begin{itemize}
        \item  Lessons from a workable solution - nutrition labeling for packaged food.

        \item Initial lessons - assessing and rating machine translators
        \item The way forward in a causal setup
    \end{itemize}

    \item Research challenges
        \begin{itemize}
        \item  Data availability: generation, sampling
        \item Assessing behavior 
        \item Assigning labels with clear  semantics 
        \item Handling composition - multiple data formats, multiple AI models 
        \item User studies on rating effectiveness
    \end{itemize}
\end{enumerate}

\subsection{Abstract of the Talk}

AI services are known to have unstable behavior when sub-
jected to changes in data, models or users. Such behaviors,
whether triggered by omission or commission, lead to trust
issues when AI work with humans. The current approach of
assessing AI services in a black box setting, where the consumer does not have access to the AI’s source code or training
data, is limited. The consumer has to rely on the AI developer’s documentation and trust that the system has been built
as stated. Further, if the AI consumer reuses the service to
build other services which they sell to their customers, the
consumer is at the risk of the service providers (both data and
model providers). Our approach, in this context, is inspired by
the success of nutritional labeling in food industry to promote
health and seeks to assess and rate AI services for trust from
the perspective of an independent stakeholder. The ratings be-
come a means to communicate the behavior of AI systems so
that the consumer is informed about the risks and can make
an informed decision. In this paper, we will first describe re-
cent progress in developing rating methods for text-based ma-
chine translator AI services that have been found promising
with user studies. Then, we will outline challenges and vision
for a principled, multi-modal, causality-based rating method-
ologies and its implication for decision-support in real-world
scenarios like health, education and food recommendation.

% --------------------
\section{CV of Biplav Srivastava}


\subsection{Employment History}
\begin{itemize}
    \item 2020-:	Professor,	AI Institute, University of South Carolina, Columbia, SC, USA



    \item 2001-2010: IBM	
   
   \begin{itemize} 
\item 2018-2020:	Distinguished Data Scientist, Master Inventor	IBM Chief Analytics Office, NY, USA

    \item 2016-2018: Research Staff Member, Master Inventor,	IBM T.J. Watson Lab, NY, USA

\item 2009-2016:	Senior Researcher, Master Inventor	IBM Research, New Delhi, India

\item 2007-2009:	Research Staff Member, IBM T.J. Watson Lab, NY, USA

\item 2001-2007:	Research Staff Member	IBM Research, Delhi \& Bangalore, India
   \end{itemize}

\item 2000-2001:	Core Technology Architect, R\&D	Bodha.com, Los Altos, CA, USA

\item 1996-2000:	Senior Staff Engineer, Philips Semi. (VLSI Tech.), Phoenix, USA; 
PhD Scholar,
Arizona State University, USA

\end{itemize}	

 	          


\subsection{Education}
\begin{itemize}
    \item Ph.D.: Arizona State University, Tempe, AZ, USA, 2000. Dissertation Topic: Efficient Planning by Effective Resource Reasoning
    \item M.S.:  Arizona State University, Tempe, AZ, USA, 1996. GPA:4.0/4.0
    \item B.Tech.: Indian Institute of Technology (IIT), B.H.U., India, 1993.  GPA:9.06/10
    \item Micro-MBA: Management module at IBM taught by faculties of top-US MBA schools.
\end{itemize}	
             
\subsection{Research Interests}
He is interested in enabling people to make rational decisions despite real world complexities of poor data, changing goals and limited resources by augmenting their cognitive limitations with technology. His expertise is in Artificial Intelligence, Sustainability and Services, with proven track record of many science firsts and high-impact innovation (\$B+) in global business environment. 
His research initiatives are on 
promoting 
goal-oriented, ethical, human-machine collaboration  via natural interfaces using  
domain and user models, learning and planning. In particular, he has been exploring the role of reasoning (planning) and learning for human-agent dialogs in individual
and group settings. The use cases are (a) explaining large datasets and their insights to people, and (b) embodiment agents
(environment or room) that can track the discussion and intervene to provide decision support to a group of people.

Biplav has been working in AI trust for 
the last four years pursuing ideas in AI testing, rating, randomized control and adversarial
learning. 
He has conducted Randomized Control Trail (RCT) tests in a large-scale business environment to study
impact of AI on workforce (involving ~140m revenue and ~1000 people; July-Dec 2019). Together with collaborators, he has introduced the idea of rating AI systems for bias as a third-party service, built tools and conducted
experiments.
He applies AI and trust techniques in areas of social as well as commercial relevance 
with particular attention to issues of developing countries  (e.g., water, health, 
transportation, and governance).
He lead building of a tool to understand the role of face mask in controlling COVID19 in US which received significant press.

\subsection{Recognition and Awards}

\begin{itemize}
    \item AAAI Senior Member, recognized by Association for Advancement of Artificial Intelligence for significant contributions and service to AI community (Feb 2020)
    \item AAAS Leshner Public Engagement Fellow, 2020-2021 cohort of the American Association for the Advancement of Science Leshner Leadership Institute for Public Engagement with Science, focusing on AI (Feb 2020)
    \item IBM Master Inventor – for outstanding patent activities (2011-2017, 2019-2022)
    \item Represented IBM at Partnership on AI’s Working Group on Fair, Transparent and Accountable AI 
(2018-2020). https://www.partnershiponai.org 
    \item IEEE Senior Member, for technical achievements (Dec 2018)
\end{itemize}

\subsection{Contributions related to the proposed topic}


\begin{itemize}
    \item Tutorial
    
    \begin{itemize}
      \item Tutorial on Trusting AI by Testing and Rating Third Party Offerings, in conjunction with 29th International Joint Conference on Artificial Intelligence (IJCAI 2020), Biplav Srivastava, Francesca Rossi, Yokohoma, Japan, Jan 2021.
    \end{itemize}
    
    \item Rating related papers
    \begin{itemize}

    
    \item  Mariana Bernagozzi, Biplav Srivastava, Francesca Rossi and Sheema Usmani, Gender Bias in Online Language Translators: Visualization, Human Perception, and Bias/Accuracy Trade-offs, IEEE Internet Computing, Special Issue on Sociotechnical Perspectives,  2021  [Visualizing Ethics Rating, User Survey]

    \item  Mariana Bernagozzi, Biplav Srivastava, Francesca Rossi and Sheema Usmani, VEGA: a Virtual Environment for Exploring Gender Bias vs. Accuracy Trade-offs in AI Translation Services, AAAI 2021. [Visualizing Ethics Rating, Demonstration paper]

    \item  Biplav Srivastava, Francesca Rossi, Sheema Usmani, and Mariana Bernagozzi, Personalized Chatbot Trustworthiness Ratings, IEEE Transactions on Technology and Society, 2020.
    %Pre-publication version on Arxiv - https://arxiv.org/abs/2005.10067, 2020. 
    [Chatbot, Trust Rating, Ethics]

    \item  Biplav Srivastava, Francesca Rossi, Rating AI Systems for Bias to Promote Trustable Applications, IBM Journal of Research and Development, 2019. [AI Service Rating, Ethics]

    \item  Biplav Srivastava, Francesca Rossi, Towards Composable Bias Rating of AI Systems, 2018 AI Ethics and Society Conference (AIES 2018), New Orleans, Louisiana, USA, Feb 2-3, 2018. [AI Service Rating, Ethics]
    \end{itemize}
    
    
    \item Closely related work
    \begin{itemize}
    
          \item Biplav Srivastava, Did Chatbots Miss Their 'Apollo Moment'? A Survey of the Potential, Gaps and Lessons from Using Collaboration Assistants During COVID-19, Cell PATTERNS, Aug 2021. 
          %(Preprint on Arxiv: https://arxiv.org/abs/2103.05561, March 2021)
          [Chatbots, COVID]
    
  
        \item 
    
    Andrea Loreggia, Nicholas Mattei, Taher Rahgooy, Francesca Rossi, Biplav Srivastava and Kristen Brent Venable, Making Human-Like Moral Decisions, AIES 2022. [Neuro-Symbolic, Fast Slow AI, Metacognition]
    
    \item Vignesh Narayanan, Brett W. Robertson, Andrea Hickerson, Biplav Srivastava and Bryant W. Smith, Securing social media for seniors from information attacks: Modeling, detecting, intervening, and communicating risks, The Third IEEE International Conference on Cognitive Machine Intelligence (IEEE CogMI), 2021. [Cyberspace, Seniors] 
    
    \item Bryant Chen, Wilka Carvalho, Nathalie Baracaldo, Heiko Ludwig, Benjamin Edwards, Taesung Lee, Ian Molloy, Biplav Srivastava, Detecting Backdoor Attacks on Deep Neural Networks by Activation Clustering, Artificial Intelligence Safety Workshop (SafeAI) at AAAI-2019, Honolulu, USA, Jan 2019. Best Paper at SafeAI 2019 Workshop. [AI-NN, Safety]
\end{itemize}
\end{itemize}

==> content/part2_paper.tex <==
\newpage

\subsection{Part II: Paper}
% --------------------
\section{Rating of Multimodal AI Systems in a Causal Setup to Communicate Trust }

\noindent {\bf Biplav Srivastava, Kausik Lakkaraju,  Mariana Bernagozzi, Marco Valtorta} \\



==> content/sec5b_sashighlights.tex <==
In summary, our approach consists of the following main steps:
% \begin{enumerate}
%     \item 
    (1) experimental apparatus consisting of data and SASs to be used, 
    %\item 
    (2) creating a causal framework,
    %\item 
    (3) performing statistical tests to assess causal dependency,
    %\item 
    (4) assigning ratings.
%\end{enumerate}
% We arrange the following sub-sections along these steps.
We now discuss them in turn.


